Magellan Adaptive Optics first-light observations of the exoplanet beta Pic b. II. 3-5 micron direct imaging with MagAO+Clio, and the empirical bolometric luminosity of a self-luminous giant planet

Young giant exoplanets are a unique laboratory for understanding cool, low-gravity atmospheres. A quintessential example is the massive extrasolar planet $\beta$ Pic b, which is 9 AU from and embedded in the debris disk of the young nearby A6V star $\beta$ Pictoris. We observed the system with first light of the Magellan Adaptive Optics (MagAO) system. In Paper I we presented the first CCD detection of this planet with MagAO+VisAO. Here we present four MagAO+Clio images of $\beta$ Pic b at 3.1 $\mu$m, 3.3 $\mu$m, $L^\prime$, and $M^\prime$, including the first observation in the fundamental CH$_4$ band. To remove systematic errors from the spectral energy distribution (SED), we re-calibrate the literature photometry and combine it with our own data, for a total of 22 independent measurements at 16 passbands from 0.99--4.8 $\mu$m. Atmosphere models demonstrate the planet is cloudy but are degenerate in effective temperature and radius. The measured SED now covers $>$80\% of the planet's energy, so we approach the bolometric luminosity empirically. We calculate the luminosity by extending the measured SED with a blackbody and integrating to find log($L_{bol}$/$L_{Sun}$) $= -3.78\pm0.03$. From our bolometric luminosity and an age of 23$\pm$3 Myr, hot-start evolutionary tracks give a mass of 12.7$\pm$0.3 $M_{Jup}$, radius of 1.45$\pm$0.02 $R_{Jup}$, and $T_{eff}$ of 1708$\pm$23 K (model-dependent errors not included). Our empirically-determined luminosity is in agreement with values from atmospheric models (typically $-3.8$ dex), but brighter than values from the field-dwarf bolometric correction (typically $-3.9$ dex), illustrating the limitations in comparing young exoplanets to old brown dwarfs.

==> figures.tex <==
%\begin{figure}
%\centering
%	%\includegraphics[height=0.49\linewidth,angle=90]{figures/bpicb_31_image_sat.eps}
%	\includegraphics[height=0.49\linewidth,angle=90]{figures/bpicb_31_image_unsat.eps}
%	%\includegraphics[height=0.49\linewidth,angle=90]{figures/bpicb_33_image_sat.eps}
%	\includegraphics[height=0.49\linewidth,angle=90]{figures/bpicb_33_image_unsat.eps}
%	%\includegraphics[height=0.49\linewidth,angle=90]{figures/bpicb_lp_image_sat.eps}
%	\includegraphics[height=0.49\linewidth,angle=90]{figures/bpicb_lp_image_unsat.eps}
%	\includegraphics[height=0.49\linewidth,angle=90]{figures/bpicb_m_image_unsat.eps}
%	\caption{\label{fig:psfs}
%	Median unsaturated PSFs.
%	Log scale images, normalized to the peak.
%	}
%\end{figure}
%
%
%\begin{figure}
%\centering
%	\includegraphics[height=0.49\linewidth,angle=90]{figures/bpicb_31_image_pca20.eps}
%	\includegraphics[height=0.49\linewidth,angle=90]{figures/bpicb_33_image_pca25.eps}
%	\includegraphics[height=0.49\linewidth,angle=90]{figures/bpicb_lp_image_pca25.eps}
%	\includegraphics[height=0.49\linewidth,angle=90]{figures/bpicb_m_image_pca20.eps}
%	\caption{\label{fig:resids}
%	Final PCA residuals.
%	Linear scale images, normalized to the peak.
%	}
%\end{figure}




%\begin{figure}
%\centering
%	\includegraphics[height=0.45\linewidth,angle=90]{figures/bpicb_31_image_unsat.eps}
%	\includegraphics[height=0.45\linewidth,angle=90]{figures/bpicb_31_image_pca20.eps}
%	\includegraphics[height=0.45\linewidth,angle=90]{figures/bpicb_33_image_unsat.eps}
%	\includegraphics[height=0.45\linewidth,angle=90]{figures/bpicb_33_image_pca25.eps}
%	\includegraphics[height=0.45\linewidth,angle=90]{figures/bpicb_lp_image_unsat.eps}
%	\includegraphics[height=0.45\linewidth,angle=90]{figures/bpicb_lp_image_pca25.eps}
%	\includegraphics[height=0.45\linewidth,angle=90]{figures/bpicb_m_image_unsat.eps}
%	\includegraphics[height=0.45\linewidth,angle=90]{figures/bpicb_m_image_pca20.eps}
%	\caption{\label{fig:psfsandresids}
%	Median unsaturated PSFs (log scale) and PCA residuals (linear scale).
%	}
%\end{figure}


